Homogenization of 2D materials in the Thomas-Fermi-von Weizsacker theory

We study the homogenization of the Thomas-Fermi-von Weizsacker (TFW) model for 2D materials. It consists in considering 2D-periodic nuclear densities with periods going to zero. We study the behavior of the corresponding ground state electronic densities and ground state energies. The main result is that these three dimensional problems converge to a limit model that is one dimensional. We also illustrate this convergence with numerical simulations and estimate the converging rate for the ground state electronic densities and the ground state energies.

==> backup.tex <==
%\section{question 25}

%Suppose in dimension $3$:
%$$\Delta \phi = f$$
%with $f\in L^1$. do we have $ \int_{\\R^3} \phi \Delta \phi = \int_{\\R^3} |\nabla \phi |^2 $?  

%we have in Fourier $ |\xi|^2 \hat \phi = \hat f$. 

%As $f$ is in $L^1$ then $\hat f$ is in $L_\infty \cap C_0$.

%Hence $\hat \phi = \frac{\hat f}{|\xi|^2}$ is $L_\infty \cap C_0$ and integrable at infinity but not arround $0$. Hence we annot say that $phi$ is $L^1$...

%We would like to proof that $\phi$ tends to zero at $\infty$ (or that $\nabla \phi$ does)

%\subsection{regularisation}

%if we take 
%$$\Delta \phi + \phi = f$$
%with $f\in L^1$. 
%do we have $ \int_{\\R^3} \phi \Delta \phi = \int_{\\R^3} |\nabla \phi |^2 $?  

%we have in fourier  $ (1+|\xi|^2) \hat \phi = \hat f$.  As $f$ is in $L^1$ then $\hat f$ is in $L_\infty \cap C_0$.

%Hence $\hat \phi = \frac{\hat f}{1+|\xi|^2}$ is $L_\infty \cap C_0$ and also $L^1$ (using $f$ in $L_\infty$).

%As $\hat \phi$ is $L^1$, hence $\phi$ ( $=\hat \hat \phi (-x)$ ) is $L^\infty \cap C_0$. Hence in intergration by parts we can drop terms at $\infty$
%$$ \int \Delta \phi \phi = \int |\nabla \phi|^2$$
% and hence $$\int |\nabla \phi|^2 + \int |\phi|^2 = \int f \phi $$

%For this take $\epsilon > 0$ and the regularized equation

%$$\Delta \phi_{\epsilon} + \epsilon \phi_{\epsilon} = f$$
%we have in fourier  $ (\epsilon +|\xi|^2) \hat \phi_{\epsilon} = \hat f$. 

%$\hat \phi = \frac{\hat f}{\epsilon +|\xi|^2}$ is $L^\infty \cap C_0$ and also $L^1$ (using $f$ in $L^\infty$). unnifom bounds in $\epsilon$ ? compacity ?

%$$ \int \Delta \phi_{\epsilon} \phi_{\epsilon} = \int |\nabla \phi_{\epsilon}|^2$$

%tending  $\epsilon$ to $0$ ?
\section{solution}


\begin{lemma} \label{lem:grad_conv_dist}
If $f_n \to f$ in $Y_{\text{per}}$, then $\Grad(G*f_n) \to \Grad(G*f)$ in $D'(\Gamma)$ (the space of distributions on $\Gamma$).
\end{lemma}
\begin{proof}
Let $\Phi_n = G*f_n$ and $\Phi = G*f$. We have $-\Laplace(\Phi_n - \Phi) = 4\pi(f_n - f)$.
Since $f_n \to f$ in $L^{5/3}(\Gamma)$, elliptic regularity implies $\Phi_n - \Phi \to 0$ in $W^{2, 5/3}_{\text{loc}}(\Gamma)$.
This means $\Grad(\Phi_n - \Phi) \to 0$ in $L^{5/3}_{\text{loc}}(\Gamma)$.
For any test function $\phi \in C^\infty_0(\Gamma)$,
$$ \abs{\int_\Gamma (\Grad\Phi_n - \Grad\Phi) \cdot \phi \, dV} \le \norm{\Grad\Phi_n - \Grad\Phi}_{L^{5/3}(\supp(\phi))} \norm{\phi}_{L^{5/2}(\supp(\phi))}. $$
As $\norm{\Grad\Phi_n - \Grad\Phi}_{L^{5/3}(\supp(\phi))} \to 0$, we have $\Grad\Phi_n \to \Grad\Phi$ in $D'(\Gamma)$.
\end{proof}


\begin{enumerate}
    \item     Let $f_0 \in Y_{\text{per}} \cap C^\infty_0(\Gamma)$ and $\Phi_0 = G*f_0$. Then $-\Laplace \Phi_0 = 4\pi f_0$.
    $$ \int_\Gamma \Phi_0 f_0 \, dV = -\frac{1}{4\pi} \int_\Gamma \Phi_0 \Laplace \Phi_0 \, dV. $$
    Using Green's first identity and the fact that boundary terms vanish for compactly supported $f_0$ (and thus sufficiently decaying $\Phi_0$):
    $$ \int_\Gamma \Phi_0 f_0 \, dV = \frac{1}{4\pi} \int_\Gamma |\Grad\Phi_0|^2 \, dV. $$
    This also implies $\Grad\Phi_0 \in L^2(\Gamma)$.

    \item  The space $Y_{\text{per}} \cap C^\infty_0(\Gamma)$ is dense in $Y_{\text{per}}$. For $f \in Y_{\text{per}}$, let $(f_n)$ be a sequence in $Y_{\text{per}} \cap C^\infty_0(\Gamma)$ such that $f_n \to f$ in $Y_{\text{per}}$.
    This implies $f_n \to f$ in $L^1(\Gamma)$ and $L^{5/3}(\Gamma)$. Let $\Phi_n = G*f_n$ and $\Phi = G*f$.
    By continuity of $h \mapsto G*h : Y_{\text{per}} \to L^\infty(\Gamma)$, we have $\Phi_n \to \Phi$ in $L^\infty(\Gamma)$.

    \item $\int_\Gamma \Phi_n f_n \, dV \to \int_\Gamma \Phi f \, dV$.
    \begin{align*}
        \abs{\int_\Gamma \Phi_n f_n \, dV - \int_\Gamma \Phi f \, dV} &\le \abs{\int_\Gamma \Phi_n (f_n - f) \, dV} + \abs{\int_\Gamma (\Phi_n - \Phi) f \, dV} \\
        &\le \norm{\Phi_n}_{L^\infty} \norm{f_n - f}_{L^1} + \norm{\Phi_n - \Phi}_{L^\infty} \norm{f}_{L^1} \to 0.
    \end{align*}

    \item 
    From step 1, $\int_\Gamma \Phi_n f_n \, dV = \frac{1}{4\pi} \norm{\Grad\Phi_n}_{L^2(\Gamma)}^2$.
    Since $\int_\Gamma \Phi_n f_n \, dV \to \int_\Gamma \Phi f \, dV$, the sequence $\norm{\Grad\Phi_n}_{L^2(\Gamma)}^2$ converges, so $\norm{\Grad\Phi_n}_{L^2(\Gamma)}$ is bounded.
    By Lemma~\ref{lem:grad_conv_dist}, $\Grad\Phi_n \to \Grad\Phi$ in $D'(\Gamma)$. Since $\norm{\Grad\Phi_n}_{L^2(\Gamma)}$ is bounded, we can extract a subsequence (still denoted $\Grad\Phi_n$) such that $\Grad\Phi_n \rightharpoonup \Grad\Phi$ weakly in $L^2(\Gamma)$.
    By weak lower semicontinuity of the $L^2$-norm (Fatou's Lemma):
    $$ \norm{\Grad\Phi}_{L^2(\Gamma)}^2 \le \liminf_{n\to\infty} \norm{\Grad\Phi_n}_{L^2(\Gamma)}^2. $$
    Thus, $\frac{1}{4\pi} \norm{\Grad\Phi}_{L^2(\Gamma)}^2 \le \lim_{n\to\infty} \frac{1}{4\pi} \norm{\Grad\Phi_n}_{L^2(\Gamma)}^2 = \int_\Gamma \Phi f \, dV$.
    This shows $\Grad\Phi \in L^2(\Gamma)$ for $f \in Y_{\text{per}}$.

    \item
    We have $-\Laplace\Phi = 4\pi f$. Multiplying by $\Phi$ and integrating:
    $$ \int_\Gamma \Phi f \, dV = -\frac{1}{4\pi} \int_\Gamma \Phi \Laplace\Phi \, dV. $$
    The following equality is true in   $Y_{\text{per}} \cap C^\infty_0(\Gamma)$ that is dense in $Y_{\text{per}}$:
    $$ \int_\Gamma (G*f) \times f \, dV = \int_\Gamma |\Grad(G*f)|^2 \, dV. $$
    We can conclude.
\end{enumerate}

